Reinforced Information Retrieval

While retrieval techniques are widely used in practice, they still face significant challenges in cross-domain scenarios. Recently, generation-augmented methods have emerged as a promising solution to this problem. These methods enhance raw queries by incorporating additional information from an LLM-based generator, facilitating more direct retrieval of relevant documents. However, existing methods struggle with highly specialized situations that require extensive domain expertise. To address this problem, we present \textbf{Reinforced-IR}, a novel approach that jointly adapts a pre-trained retriever and generator for precise cross-domain retrieval. A key innovation of Reinforced-IR is its \textbf{Self-Boosting} framework, which enables retriever and generator to learn from each other's feedback. Specifically, the generator is reinforced to generate query augmentations that enhance the retriever's performance, while the retriever is trained to better discriminate the relevant documents identified by the generator. This iterative process allows the end-to-end retrieval performance to be progressively optimized using an unlabeled corpus from the target domain. In our experiment, Reinforced-IR outperforms existing domain adaptation methods by a large margin, leading to substantial improvements in retrieval quality across a wide range of application scenarios.

==> exp.tex <==
\definecolor{darkgreen}{rgb}{0.0, 0.65, 0.0}

\begin{table*}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l|ccccccccc|cccccc|c}
        \toprule
         & \multicolumn{9}{c|}{BEIR} & \multicolumn{6}{c|}{AIR-Bench} & \multirow{2}{*}{\textbf{AVG}} \\
        \cmidrule(lr){2-10} \cmidrule(lr){11-16}
         & FiQA & Scidocs & FEVER & Arguana & Scifact & TREC-COVID & Touche & DBPedia & \textbf{avg} & law & news & healthcare & finance & arxiv & \textbf{avg} & \\
        \midrule
        \multicolumn{17}{l}{Contriever} \\
        \midrule
        % BM25 & 23.6 & 15.8 & 75.3 & 31.5 & 66.5 & 65.6 & 36.7 & 31.3 & 43.3 & 18.3 & 46.8 & 38.5 & 41.1 & 31.5 & 35.2 & 40.2 \\
        Contriever & 24.5 & 14.9 & 68.2 & 37.9 & 64.9 & 27.3 & 16.7 & 29.2 & 35.4 & 2.3 & 16.9 & 27.1 & 25.3 & 11.3 & 16.6 & 28.2 \\
        % Contriever-ft & 32.9 & 16.5 & 75.8 & 44.6 & 67.7 & 59.6 & 20.4 & 41.3 & 44.9 & 9.1 & 36.2 & 41.3 & 37.3 & 27.1 & 30.2 & 39.2 \\
        \midrule
        HyDE & 26.2 & 12.4 & 69.5 & 40.9 & 66.5 & 59.7 & 15.8 & 33.9 & 40.6 & 1.4 & 15.1 & 31.8 & 18.6 & 11.4 & 15.7 & 31.0 \\
        Doc2query & 25.5 & 15.3 & 69.4 & 39.5 & 65.9 & 29.2 & 12.6 & 29.9 & 35.9 & 2.9 & 17.3 & 28.5 & 27.6 & 12.4 & 17.7 & 28.9 \\
        QGen & 31.6 & 17.8 & 66.9 & 50.1 & 69.0 & 63.3 & 19.0 & 34.3 & 44.0 & 22.5 & 32.3 & 35.2 & 36.2 & 24.8 & 30.2 & 38.7 \\
        GPL & 33.2 & 17.7 & 77.5 & 44.5 & 58.4 & 67.1 & 21.6 & 42.7 & 45.3 & 22.0 & 39.9 & 40.9 & 35.3 & 30.4 & 33.7 & 40.9 \\
        IR-Studio & 36.8 & 19.2 & 81.3 & 52.6 & 70.9 & 78.6 & 31.1 & 47.5 & 52.3 & 28.3 & 43.8 & 43.2 & 40.7 & 33.4 & 37.9 & 46.7 \\
        \midrule
        \multicolumn{17}{l}{BGE-M3} \\
        \midrule
        BGE-M3 & 41.1 & 16.4 & 81.0 & 54.1 & 64.2 & 54.7 & 22.3 & 39.8 & 46.7 & 25.6 & 50.8 & 49.1 & 46.0 & 37.4 & 41.8 & 44.8 \\
        \midrule
        HyDE & 39.2 & 16.9 & 75.8 & 53.2 & 67.2 & 71.7 & 19.6 & 42.5 & 48.3 & 20.7 & 45.6 & 44.1 & 42.7 & 31.6 & 36.9 & 43.9 \\
        Doc2query & 37.7 & 16.8 & 74.8 & 56.0 & 64.3 & 39.4 & 14.0 & 39.5 & 42.8 & 23.8 & 48.4 & 44.7 & 45.7 & 37.8 & 40.1 & 41.8 \\
        QGen & 41.8 & 18.3 & 80.3 & 65.6 & 67.8 & 70.1 & 22.1 & 41.4 & 50.9 & 32.2 & 50.7 & 45.3 & 48.3 & 38.2 & 42.9 & 47.9 \\
        GPL & 43.2 & 18.7 & 79.1 & 65.5 & 65.3 & 74.6 & 24.1 & 41.5 & 51.5 & 27.5 & 50.6 & 51.0 & 45.6 & 37.7 & 42.5 & 48.0 \\
        IR-Studio & 45.8 & 19.2 & 84.7 & 65.1 & 68.2 & 83.9 & 32.4 & 45.5 & 55.6 & 32.5 & 52.6 & 51.5 & 48.9 & 39.7 & 45.0 & 51.5 \\
        \bottomrule
    \end{tabular}%
    }
    \vspace{0.1cm}
    \caption{The overall performance (nDCG@10 [\%]) on the BEIR and AIR-Bench benchmarks.}
    \label{overall}
\end{table*}

\begin{table*}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l|ccccccccc|cccccc|c}
        \toprule
         & \multicolumn{9}{c|}{BEIR} & \multicolumn{6}{c|}{AIR-Bench} & \multirow{2}{*}{\textbf{AVG}} \\
        \cmidrule(lr){2-10} \cmidrule(lr){11-16}
         & FiQA & Scidocs & FEVER & Arguana & Scifact & TREC-COVID & Touche & DBPedia & \textbf{avg} & law & news & healthcare & finance & arxiv & \textbf{avg} & \\
        \midrule
        Contriever & 24.5 & 14.9 & 68.2 & 37.9 & 64.9 & 27.3 & 16.7 & 29.2 & 35.4 & 2.3 & 16.9 & 27.1 & 25.3 & 11.3 & 16.6 & 28.2 \\
        \midrule
        w/ RLRF & 28.5 & 15.4 & 74.6 & 40.2 & 66.7 & 41.4 & 19.3 & 34.9 & 40.1 & 2.7 & 17.7 & 30.7 & 24.2 & 12.6 & 17.6 & 31.5 \\
        w/ RLGF & 35.6 & 19.1 & 75.7 & 52.7 & 70.6 & 74.7 & 27.9 & 45.7 & 50.3 & 25.1 & 43.6 & 42.5 & 39.9 & 32.3 & 36.7 & 45.0 \\
        w/ RLRF \& RLGF & 36.8 & 19.2 & 81.3 & 52.6 & 70.9 & 78.6 & 31.1 & 47.5 & 52.3 & 28.3 & 43.8 & 43.2 & 40.7 & 33.4 & 37.9 & 46.7 \\
        \bottomrule
    \end{tabular}%
    }
    \vspace{0.1cm}
    \caption{The performance of each technology on the BEIR and AIR-Bench benchmarks.}
    \label{technology}
\end{table*}

\begin{table*}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l|cccccccc|c|ccccc|c}
        \toprule
         & \multicolumn{9}{c|}{BEIR} & \multicolumn{6}{c}{AIR-Bench} \\
        \cmidrule(lr){2-10} \cmidrule(lr){11-16}
         & FiQA & Scidocs & Fever & Argu. & Scifact & T-Covid & Touche & DBPedia & \textbf{AVG} & Law & News & Health & Fin. & ArXiv & \textbf{AVG} \\ 
        \midrule
        Contriever & 24.5 & 14.9 & 68.2 & 37.9 & 64.9 & 27.3 & 16.7 & 29.2 & 35.5 & 2.3 & 16.9 & 27.1 & 25.3 & 11.3 & 16.6 \\
        HyDE (Mist, Ctrv) & 25.3 & 12.4 & 69.5 & 38.6 & 69.2 & 55.0 & 19.7 & 35.8 & 40.7 & 1.9 & 15.5 & 30.6 & 18.8 & 11.8 & 15.7 \\
        HyDE (Qwen, Ctrv) & 24.6 & 13.2 & 63.1 & 39.0 & 68.2 & 52.1 & 17.8 & 31.6 & 38.7 & 1.5 & 13.1 & 29.7 & 19.2 & 11.5 & 15.0 \\
        HyDE (Llama, Ctrv) & 26.2 & 12.4 & 69.5 & 40.9 & 66.5 & 59.7 & 15.8 & 33.9 & 40.6 & 1.4 & 15.1 & 31.8 & 18.6 & 11.4 & 15.7 \\
        Ours (Mist, Ctrv) & \textbf{38.0} & \textbf{19.5} & 81.0 & 52.4 & 70.5 & 78.3 & 30.6 & \textbf{47.5} & 52.2 & 27.1 & \textbf{44.1} & \textbf{43.3} & 39.1 & 31.8 & 37.1 \\
        Ours (Qwen, Ctrv) & 36.7 & 19.4 & 78.2 & 52.0 & \textbf{71.1} & 75.7 & \textbf{31.2} & 46.2 & 51.3 & 27.0 & 42.8 & 43.0 & 38.5 & \textbf{33.6} & 37.0 \\
        Ours (Llama, Ctrv) & 36.8 & 19.2 & \textbf{81.3} & \textbf{52.6} & 70.9 & \textbf{78.6} & 31.1 & \textbf{47.5} & \textbf{52.3} & \textbf{28.3} & 43.8 & 43.2 & \textbf{40.7} & 33.4 & \textbf{37.9} \\
        \midrule
        SimLM & 17.7 & 11.9 & 31.7 & 34.3 & 49.2 & 40.7 & 9.8 & 33.1 & 28.6 & 1.8 & 15.3 & 41.0 & 32.7 & 17.8 & 21.7 \\
        HyDE (Llama, Sim) & 20.5 & 12.9 & 39.5 & 34.4 & 52.3 & 58.9 & 16.4 & 39.1 & 34.2 & 8.3 & 18.1 & 39.0 & 30.6 & 17.1 & 21.1 \\
        Ours (Llama, Sim) & \textbf{35.0} & \textbf{18.3} & \textbf{77.8} & \textbf{58.7} & \textbf{66.3} & \textbf{74.3} & \textbf{29.7} & \textbf{43.1} & \textbf{50.4} & \textbf{25.3} & \textbf{43.7} & \textbf{47.7} & \textbf{41.6} & \textbf{34.6} & \textbf{38.6} \\
        \midrule
        Retromae & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        HyDE (Llama, Retro) & 26.4 & 13.7 & 75.9 & 37.4 & 62.8 & 72.0 & 25.4 & 38.1 & 44.0 & 9.7 & 38.8 & 36.1 & 29.2 & 22.3 & 27.2 \\
        Ours (Llama, Retro) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        \midrule
        Contriever-ft & 32.9 & 16.5 & 75.8 & 44.6 & 67.7 & 59.6 & 20.4 & 41.3 & 44.9 & 9.1 & 36.2 & 41.3 & 37.3 & 27.1 & 30.2 \\
        HyDE (Llama, C-ft) & 31.2 & 15.8 & 77.4 & 40.6 & 67.7 & 72.9 & 26.6 & 41.8 & 46.8 & 8.6 & 38.9 & 39.6 & 34.5 & 24.5 & 29.2 \\
        Ours (Llama, C-ft) & \textbf{38.7} & \textbf{18.7} & \textbf{84.4} & \textbf{52.1} & \textbf{70.4} & \textbf{78.5} & \textbf{34.3} & \textbf{46.4} & \textbf{52.9} & \textbf{28.6} & \textbf{44.3} & \textbf{46.6} & \textbf{40.4} & \textbf{35.1} & \textbf{39.0} \\
        \midrule
        gte-large & 44.6 & 23.4 & \textbf{84.5} & 57.3 & \textbf{74.3} & 70.2 & 25.5 & 42.4 & 52.8 & 16.1 & 46.0 & 51.5 & 43.0 & 36.7 & 38.9 \\
        HyDE (Llama, gte) & 43.5 & \textbf{23.6} & 81.0 & 53.9 & 75.4 & 75.5 & 22.5 & 44.8 & 52.5 & 13.6 & 44.5 & 47.6 & 40.5 & 34.3 & 36.1 \\
        Ours (Llama, gte) & \textbf{46.1} & 23.2 & 84.1 & \textbf{66.8} & 73.8 & \textbf{84.8} & \textbf{31.7} & \textbf{47.3} & \textbf{57.2} & \textbf{30.3} & \textbf{52.8} & \textbf{56.4} & \textbf{48.3} & \textbf{42.7} & \textbf{46.1} \\
        \midrule
        stella-base-en-v2 & 38.6 & 18.6 & 79.1 & 60.7 & 72.5 & 64.7 & 21.9 & 39.7 & 49.5 & 15.9 & 42.7 & 50.0 & 40.7 & 30.4 & 36.0 \\
        HyDE (Llama, stella) & 37.8 & 21.2 & 71.5 & 55.1 & 73.6 & 80.4 & 25.3 & 42.2 & 50.9 & 13.3 & 43.3 & 46.4 & 39.2 & 30.8 & 34.6 \\
        Ours (Llama, stella) & \textbf{43.7} & \textbf{22.3} & \textbf{84.2} & \textbf{64.7} & \textbf{74.1} & \textbf{84.2} & \textbf{30.1} & \textbf{45.4} & \textbf{56.1} & \textbf{27.3} & \textbf{49.4} & \textbf{53.2} & \textbf{47.1} & \textbf{37.8} & \textbf{43.0} \\
        \midrule
        BGE-M3 & 41.1 & 16.4 & 81.0 & 54.1 & 64.2 & 54.7 & 22.3 & 39.8 & 46.7 & 25.6 & 50.8 & 49.1 & 46.0 & 37.4 & 41.8 \\
        HyDE (Llama, M3) & 39.2 & 16.9 & 75.8 & 53.2 & 67.2 & 71.7 & 19.6 & 42.5 & 48.3 & 20.7 & 45.6 & 44.1 & 42.7 & 31.6 & 36.9 \\
        Ours (Llama, M3) & \textbf{45.8} & \textbf{19.2} & \textbf{84.7} & \textbf{65.1} & \textbf{68.2} & \textbf{83.9} & \textbf{32.4} & \textbf{45.5} & \textbf{55.6} & \textbf{32.5} & \textbf{52.6} & \textbf{51.5} & \textbf{48.9} & \textbf{39.7} & \textbf{45.0} \\
        \bottomrule
    \end{tabular}%
    }
    \vspace{0.1cm}
    \caption{The performance (nDCG@10 [\%]) of different backbones on the BEIR and AIR-Bench benchmarks.}
    \label{backbone}
\end{table*}


\begin{table*}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l|ccccccccc|cccccc|c}
        \toprule
         & \multicolumn{9}{c|}{BEIR} & \multicolumn{6}{c|}{AIR-Bench} & \multirow{2}{*}{\textbf{AVG}} \\
        \cmidrule(lr){2-10} \cmidrule(lr){11-16}
         & FiQA & Scidocs & FEVER & Arguana & Scifact & TREC-COVID & Touche & DBPedia & \textbf{avg} & law & news & healthcare & finance & arxiv & \textbf{avg} & \\
        \midrule
        \multicolumn{17}{l}{Contriever} \\
        \midrule
        \multicolumn{17}{l}{HyDE} \\
        Contriever & 24.5 & 14.9 & 68.2 & 37.9 & 64.9 & 27.3 & 16.7 & 29.2 & 35.4 & 2.3 & 16.9 & 27.1 & 25.3 & 11.3 & 16.6 & 28.2 \\
        w/ Llama3-8B-it & 26.2 & 12.4 & 69.5 & 40.9 & 66.5 & 59.7 & 15.8 & 33.9 & 40.6 & 1.4 & 15.1 & 31.8 & 18.6 & 11.4 & 15.7 & 31.0 \\
        w/ Llama3-70B-it & 28.1 & 14.6 & 74.4 & 40.6 & 69.6 & 51.1 & 19.7 & 36.0 & 41.8 & 1.5 & 15.3 & 30.8 & 19.3 & 12.2 & 15.8 & 31.8 \\
        w/ Qwen2.5-72B-it & 25.5 & 14.1 & 77.7 & 46.6  & 70.1  & 56.8  & 18.3 & 35.1 & 43.0 & 1.5  & 12.9 & 28.0  & 17.8  & 10.8  & 14.2 & 31.9 \\
        w/ GPT-4o-mini & 26.1 & 13.2 & 76.7 & 44.4 & 68.2 & 57.3 & 18.8 & 33.4 & 42.3 & 1.8 & 15.1 & 29.7 & 21.5 & 12.1 & 16.0 & 32.2 \\
        \midrule
        \multicolumn{17}{l}{QGen + HyDE} \\
        QGen & 31.6 & 17.8 & 66.9 & 50.1 & 69.0 & 63.3 & 19.0 & 34.3 & 44.0 & 22.5 & 32.3 & 35.2 & 36.2 & 24.8 & 30.2 & 38.7 \\
        w/ Llama3-8B-it & 34.5 & 17.0 & 70.9 & 49.9 & 68.2 & 69.3 & 21.2 & 38.1 & 46.1 & 17.5 & 28.6 & 35.4 & 29.5 & 22.3 & 26.7 & 38.6 \\
        w/ Llama3-70B-it & 35.9 & 18.3 & 75.9 & 51.1 & 72.8 & 69.8 & 24.1 & 40.5 & 48.6 & 18.9 & 29.8 & 35.8 & 31.1 & 23.2 & 27.8 & 40.6 \\
        w/ Qwen2.5-72B-it & 35.7 & 18.0 & 79.3 & 55.1 & 72.4 & 71.0 & 22.6 & 38.4 & 49.1  & 17.8 & 26.2 & 32.5 & 27.3 & 21.8 & 25.1  & 39.9 \\
        w/ GPT-4o-mini & 35.8 & 17.5 & 78.4 & 53.4 & 71.2 & 70.3 & 23.8 & 36.7 & 48.4  & 18.7 & 30.2 & 34.6 & 31.2 & 23.3 & 27.6  & 40.4 \\
        \midrule
        \multicolumn{17}{l}{GPL + HyDE} \\
        GPL & 33.2 & 17.7 & 77.5 & 44.5 & 58.4 & 67.1 & 21.6 & 42.7 & 45.3 & 22.0 & 39.9 & 40.9 & 35.3 & 30.4 & 33.7 & 40.9 \\
        w/ Llama3-8B-it & 35.0 & 17.3 & 76.6 & 42.3 & 57.3 & 74.9 & 25.1 & 42.3 & 46.4 & 15.6 & 36.9 & 39.2 & 27.2 & 26.5 & 29.1 & 39.7 \\
        w/ Llama3-70B-it & 36.3 & 18.4 & 80.9 & 42.9 & 62.9 & 73.7 & 29.0 & 44.1 & 48.5 & 17.7 & 38.1 & 39.7 & 29.1 & 28.9 & 30.7 & 41.7 \\
        w/ Qwen2.5-72B-it & 35.9 & 18.5 & 83.2 & 47.1 & 63.9 & 73 & 25.6 & 41.3 & 48.6  & 16.1 & 32.7 & 36.9 & 26.4 & 27.3 & 27.9  & 40.6 \\
        w/ GPT-4o-mini & 35.2 & 17.5 & 83.2 & 44.9 & 63.3 & 73.7 & 27.6 & 40.9 & 48.3 & 17.1 & 37.2 & 39.2 & 29.7 & 28.2 & 30.3 & 41.4 \\
        \midrule
        \multicolumn{17}{l}{IR Studio} \\
        w/o Llama3-8B-it & 35.5 & 18.7 & 72.8 & 51.5 & 68.8 & 70.4 & 27.9 & 43.1 & 48.6 & 25.3 & 39.0 & 37.2 & 37.9 & 28.8 & 33.6 & 42.8 \\
        w/ Llama3-8B-it & 36.8 & 19.2 & 81.3 & 52.6 & 70.9 & 78.6 & 31.1 & 47.5 & 52.3 & 28.3 & 43.8 & 43.2 & 40.7 & 33.4 & 37.9 & 46.7 \\
        \midrule
        \multicolumn{17}{l}{BGE-M3} \\
        \midrule
        \multicolumn{17}{l}{HyDE} \\
        BGE-M3 & 41.1 & 16.4 & 81.0 & 54.1 & 64.2 & 54.7 & 22.3 & 39.8 & 46.7 & 25.6 & 50.8 & 49.1 & 46.0 & 37.4 & 41.8 & 44.8 \\
        w/ Llama3-8B-it & 39.2 & 16.9 & 75.8 & 53.2 & 67.2 & 71.7 & 19.6 & 42.5 & 48.3 & 20.7 & 45.6 & 44.1 & 42.7 & 31.6 & 36.9 & 43.9 \\
        w/ Llama3-70B-it & 40.9 & 17.5 & 80.8 & 54.4 & 70.2 & 68.9 & 22.5 & 43.6 & 49.9 & 22.1 & 46.2 & 44.2 & 40.7 & 32.8 & 37.2 & 45.0 \\
        w/ Qwen2.5-72B-it & 40.6 & 16.9 & 83.9 & 55.1 & 71.2 & 68.6 & 20.8 & 42.9 & 50.0 & 20.9 & 39.5 & 41.9 & 36.2 & 30.4 & 33.8 & 43.8 \\
        w/ GPT-4o-mini & 40.3 & 16.9 & 83.9 & 52.7 & 69.5 & 72.4 & 21.7 & 42.8 & 50.0 & 22.9 & 44.7 & 44.8 & 41.1 & 31.9 & 37.1 & 45.0 \\
        \midrule
        \multicolumn{17}{l}{QGen + HyDE} \\
        QGen & 41.8 & 18.3 & 80.3 & 65.6 & 67.8 & 70.1 & 22.1 & 41.4 & 50.9 & 32.2 & 50.7 & 45.3 & 48.3 & 38.2 & 42.9 & 47.9 \\
        w/ Llama3-8B-it & 42.0 & 19.2 & 75.7 & 60.4 & 68.6 & 78.6 & 22.1 & 42.4 & 51.1 & 27.8 & 46.2 & 40.7 & 46.5 & 31.5 & 38.5 & 46.3 \\
        w/ Llama3-70B-it & 43.8 & 19.8 & 79.6 & 62.9 & 71.9 & 75.6 & 26.4 & 43.5 & 52.9 & 28.0 & 45.8 & 42.2 & 44.4 & 33.3 & 38.7 & 47.5 \\
        w/ Qwen2.5-72B-it & 42.3 & 20.0 & 82.9 & 60.4 & 71.1 & 74.5 & 25.9 & 43.0 & 52.5 & 21.0  & 39.3 & 42.0  & 36.8 & 31.1 & 34.0 & 45.4 \\
        w/ GPT-4o-mini & 42.7 & 19.5 & 83.1 & 57.5 & 71.1 & 81.0 & 28.4 & 42.4 & 53.2 & 22.7 & 44.6 & 45.2 & 40.0 & 31.8 & 36.9 & 46.9 \\
        \midrule
        \multicolumn{17}{l}{GPL + HyDE} \\
        GPL & 43.2 & 18.7 & 79.1 & 65.5 & 65.3 & 74.6 & 24.1 & 41.5 & 51.5 & 27.5 & 50.6 & 51.0 & 45.6 & 37.7 & 42.5 & 48.0 \\
        w/ Llama3-8B-it & 40.8 & 19.4 & 75.6 & 58.0 & 67.4 & 78.3 & 23.4 & 42.4 & 50.7 & 20.5 & 44.9 & 44.7 & 41.3 & 30.5 & 36.4 & 45.2 \\
        w/ Llama3-70B-it & 42.8 & 20.4 & 79.9 & 60.4 & 70.3 & 77.7 & 28.7 & 44.0 & 53.0 & 22.4 & 45.1 & 45.0 & 40.8 & 32.4 & 37.1 & 46.9 \\
        w/ Qwen2.5-72B-it & 39.2 & 20.0 & 75.6 & 60.3 & 63.8 & 69.0 & 25.4 & 42.5 & 49.5 & 21.3 & 39.7 & 41.6 & 36.0 & 31.2 & 34.0 & 43.5 \\
        w/ GPT-4o-mini & 40.2 & 19.6 & 74.3 & 57.2 & 68.1 & 74.3 & 27.2 & 42.6 & 50.4 & 22.6 & 44.9 & 44.7 & 40.3 & 32.0 & 36.9 & 45.2 \\
        \midrule
        \multicolumn{17}{l}{IR Studio} \\
        w/o Llama3-8B-it & 44.0 & 18.9 & 81.1 & 65.4 & 67.1 & 81.2 & 30.9 & 42.2 & 53.9 & 32.5 & 50.2 & 49.7 & 48.5 & 38.3 & 43.8 & 50.0 \\
        w/ Llama3-8B-it & 45.8 & 19.2 & 84.7 & 65.1 & 68.2 & 83.9 & 32.4 & 45.5 & 55.6 & 32.5 & 52.6 & 51.5 & 48.9 & 39.7 & 45.0 & 51.5 \\
        \bottomrule
    \end{tabular}%
    }
    \vspace{0.1cm}
    \caption{The results of utilizing different LLMs on the BEIR and AIR-Bench benchmarks.}
    \label{compare}
\end{table*}

% \begin{table*}[ht]
%     \centering
%     % \resizebox{\linewidth}{!}{%
%     \begin{tabular}{l|ccccc|c}
%         \toprule
%          % & \multicolumn{6}{c|}{AIR-Bench} \\
%         % \cmidrule(lr){2-7}
%          & law & news & healthcare & finance & arxiv & \textbf{avg} \\
%         \midrule
%         IR Studio & 28.3 & 43.8 & 43.2 & 40.7 & 33.4 & 37.9 \\
%         \midrule
%         \quad w/o dpo & 23.5 & 43.5 & 42.9 & 38.7 & 32.4 & 36.2 \\
%         \quad w/o proximity & 24.4 & 41.1 & 40.2 & 37.6 & 31.6 & 35.0 \\
%         \quad w/o distill & 28.3 & 37.1 & 41.5 & 38.2 & 31.3 & 35.3 \\
%         \quad w/o sep & 25.7 & 42.9 & 41.8 & 36.5 & 29.2 & 35.2 \\
%         \bottomrule
%     \end{tabular}%
%     % }
%     \vspace{0.1cm}
%     \caption{The ablation study on the BEIR and AIR-Bench benchmarks.}
%     \label{ablation}
% \end{table*}

\begin{table*}[ht]
    \centering
    % \resizebox{\linewidth}{!}{%
    \small
    \begin{tabular}{l|cc|c}
        \toprule
         % & \multicolumn{6}{c|}{AIR-Bench} \\
        % \cmidrule(lr){2-7}
         & BEIR & AIR-Bench & \textbf{avg} \\
        \midrule
        IR Studio & 52.3 & 37.9 & 46.7 \\
        \midrule
        \quad w/o sep & 52.8 & 35.2 & 46.0 \\
        \quad w/o dpo & 50.6 & 36.2 & 45.1 \\
        \quad w/o dpo-rule1 & 49.0 & 38.0 & 44.8 \\
        \quad w/o dpo-rule2 & 49.7 & 37.4 & 45.0 \\
        \quad w/o proximity & 52.3 & 35.0 & 45.6 \\
        \quad w/o distill & 49.3 & 35.3 & 43.9 \\
        \bottomrule
    \end{tabular}%
    % }
    \vspace{0.1cm}
    \caption{The ablation study on the BEIR and AIR-Bench benchmarks.}
    \label{ablation}
\end{table*}

\begin{table*}[h]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ll|ccccccccc|cccccc|c}
        \toprule
        & & \multicolumn{9}{c|}{BEIR} & \multicolumn{6}{c|}{AIR-Bench} & \multirow{2}{*}{\textbf{AVG}} \\
        \cmidrule(lr){3-11} \cmidrule(lr){12-17}
        Ret. & Gen. & FiQA & Scidocs & FEVER & Arguana & Scifact & TREC-COVID & Touche & DBPedia & \textbf{avg} & law & news & healthcare & finance & arxiv & \textbf{avg} & \\
        \midrule
        Raw & - & 24.5 & 14.9 & 68.2 & 37.9 & 64.9 & 27.3 & 16.7 & 29.2 & 35.4 & 2.3  & 16.9 & 27.1 & 25.3 & 11.3 & 16.6 & 28.2 \\
        Raw & Raw & 27.8 & 15.4 & 72.8 & 40.5 & 67.2 & 36.6 & 18.4 & 33.7 & 39.1 & 2.1 & 17.4 & 29.4 & 25.0 & 12.1 & 17.2 & 30.6 \\
        Ret. & Gen.-1 & 28.9 & 15.6 & 74.0 & 40.3 & 67.1 & 42.9 & 20.3 & 34.9 & 40.5 & 2.5 & 17.5 & 30.6 & 23.6 & 12.6 & 17.4 & 31.6 \\
        Ret.-1 & Gen.-1 & 29.8 & 17.6 & 72.2 & 43.2 & 69.8 & 64.6 & 25.3 & 35.1 & 44.7 & 12.3 & 31.7 & 34.9 & 28.4 & 21.0 & 25.7 & 37.4 \\
        Ret.-1 & Gen.-2 & 30.8 & 17.7 & 74.9 & 42.6 & 69.9 & 69.4 & 25.2 & 35.7 & 45.8 & 15.2 & 33.7 & 35.7 & 28.8 & 22.1 & 27.1 & 38.6 \\
        Ret.-2 & Gen.-2 & 33.5 & 18.8 & 78.2 & 49.1 & 70.4 & 74.8 & 30.4 & 43.9 & 49.9 & 24.2 & 42.4 & 40.7 & 35.7 & 30.7 & 34.7 & 44.1 \\
        Ret.-2 & Gen.-3 & 33.6 & 19.1 & 79.1 & 49.7 & 70.5 & 73.6 & 31.0 & 45.2 & 50.2 & 24.7 & 42.4 & 40.9 & 37.0 & 30.8 & 35.2 & 44.4 \\
        Ret.-3 & Gen.-3 & 36.8 & 19.2 & 81.3 & 52.6 & 70.9 & 78.8 & 31.1 & 47.5 & 52.3 & 28.3 & 43.8 & 43.2 & 40.7 & 33.4 & 37.9 & 46.7 \\
        \bottomrule
    \end{tabular}%
    }
    \vspace{0.1cm}
    \caption{The performance (nDCG@10 [\%]) on the BEIR and AIR-Bench benchmarks with the iterative joint training process.}
    \label{iteration}
\end{table*}


\begin{table*}[ht]
    \centering
    \small
    \begin{tabularx}{\textwidth}{c|X} % 'X' takes up rest of space
        \toprule
        Query & Watertown, Massachusetts is in the United Kingdom. \\ \midrule
        Candidates & \textbf{\textcolor{darkgreen}{[pos] [1]}} Watertown, Massachusetts The Town of Watertown is a city in Middlesex County, Massachusetts, United States. It is part of the Greater Boston area. The population was 31,915 at the 2010 census. Watertown is one of fourteen Massachusetts municipalities that have applied for, and been granted, city forms of government but wish to retain ``The town of'' in their official names. Watertown is made up of six neighborhoods: Bemis, Brigham (Brigham Historic District), Coolidge Square, East Watertown, Watertown Square and the West End. \\ 
        & \textbf{\textcolor{red}{[neg] [2]}} Watertown High School Watertown High School may refer to: Watertown High School (Connecticut) in Watertown, Connecticut  Watertown High School (Massachusetts) in Watertown, Massachusetts  Watertown High School (New York) in Watertown, New York  Watertown High School (South Dakota) in Watertown, South Dakota  Watertown High School (Tennessee) in Watertown, Tennessee  Watertown High School (Wisconsin) in Watertown, Wisconsin \\ 
        & \textbf{\textcolor{red}{[neg] [3]}} Abe Brown Abe Brown or Abraham Brown or variant, may refer to:  Abe Brown (Marvel Comics) or Abraham Brown, a martial artist in the Marvel Universe  President Abraham Brown, a fictional president of the United States  Young Brown, or Abe Brown (born September 24, 1893, date of death unknown), was a welterweight boxer from New York City  Barnacle Bill (song), a song originating as the folk song ``Abraham Brown''  Abraham Browne House, colonial era house in Watertown, Massachusetts, USA \\ 
        & \textbf{\textcolor{red}{[neg] [4]}} Waterville Waterville is the name of several places. In Russia Waterville Aquapark, a water park attached to the Park Inn Pribaltiyskaya Hotel, Saint Petersburg In the United States: Waterville, Iowa Waterville, Kansas Waterville, Maine Waterville, Minnesota Waterville, New York Waterville, Ohio Waterville, Pennsylvania Waterville, Vermont Waterville, Washington Waterville, Wisconsin Waterville (Waterbury), a neighborhood in Connecticut Waterville USA, a water and amusement park in Alabama In Canada: Waterville, Quebec Waterville, Nova Scotia Waterville, New Brunswick (disambiguation) Waterville, Newfoundland and Labrador In Ireland: Waterville, County Kerry Waterville, Dublin \\
        & \textbf{\textcolor{red}{[neg] [5]}} Watertown Historic District Watertown Historic District or Watertown Commercial Historic District may refer to: in the United States (by state) Watertown Center Historic District, Watertown, CT, listed on the NRHP in Connecticut Watertown Arsenal Historic District, Watertown, MA, listed on the NRHP in Massachusetts Watertown Historic District (Watertown, Ohio), listed on the NRHP in Ohio Watertown Commercial Historic District (Jefferson, South Dakota), listed on the NRHP in South Dakota Watertown Commercial Historic District (Watertown, Tennessee), listed on the NRHP in Tennessee \\ \midrule \midrule
        Llama3 info. & The claim that Watertown, Massachusetts is in the United Kingdom is FALSE. \\ \midrule
        Llama3-dpo info. & The claim "Watertown, Massachusetts is in the United Kingdom" is false. Watertown is a town located in Middlesex County, Massachusetts, United States. It was incorporated as a town on August 16, 1630, and has been part of the state of Massachusetts since its founding.\newline
        According to the official website of the Town of Watertown, Massachusetts, it is situated approximately 10 miles northwest of downtown Boston and is bordered by Cambridge, Belmont, Waltham, Weston, Lincoln, and Arlington. The town's zip code is 02472, which is a US postal code.\newline
        Additionally, various online sources such as Wikipedia, TripAdvisor, and other travel websites all confirm that Watertown, Massachusetts is a town located in the United States, not in the United Kingdom. These sources provide information about the town's history, demographics, attractions, and amenities, all of which are consistent with its location in Massachusetts, USA.\newline
        Therefore, based on the available evidence, it can be concluded that the claim "Watertown, Massachusetts is in the United Kingdom" is incorrect. \\
        \midrule \midrule
        Contriever & \textbf{\textcolor{red}{[2]}} > \textbf{\textcolor{red}{[4]}} > \textbf{\textcolor{red}{[5]}} > \textbf{\textcolor{red}{[3]}} > \textbf{\textcolor{darkgreen}{[1]}} \\ \midrule
        Contriever \textbullet{} Llama3 & \textbf{\textcolor{red}{[2]}} > \textbf{\textcolor{red}{[4]}} > \textbf{\textcolor{red}{[5]}} > \textbf{\textcolor{darkgreen}{[1]}} > \textbf{\textcolor{red}{[3]}} \\ \midrule
        Contriever \textbullet{} Llama3-dpo & \textbf{\textcolor{red}{[2]}} > \textbf{\textcolor{red}{[4]}} > \textbf{\textcolor{darkgreen}{[1]}} > \textbf{\textcolor{red}{[5]}} > \textbf{\textcolor{red}{[3]}} \\ \midrule
        Contriever-st \textbullet{} Llama3 & \textbf{\textcolor{red}{[2]}} > \textbf{\textcolor{darkgreen}{[1]}} > \textbf{\textcolor{red}{[4]}} > \textbf{\textcolor{red}{[5]}} > \textbf{\textcolor{red}{[3]}} \\ \midrule
        Contriever-st \textbullet{} Llama3-dpo & \textbf{\textcolor{darkgreen}{[1]}} > \textbf{\textcolor{red}{[2]}} > \textbf{\textcolor{red}{[4]}} > \textbf{\textcolor{red}{[5]}} > \textbf{\textcolor{red}{[3]}} \\
        \bottomrule
    \end{tabularx}
    \label{case}
    \caption{The analysis of the retrieval case.}
\end{table*}

\begin{table*}[ht]
    \centering
    \small
    \begin{tabularx}{\textwidth}{c|X} % 'X' takes up rest of space
        \toprule
        Query & Assess how Italy's lower discount rate affects local bank earnings. \\ \midrule
        Candidates & \textbf{\textcolor{darkgreen}{[pos] [1]}} Italy's average interbank rate rose to a provisional 12.18 pct in February from 12.05 pct in January, figures from the Bank of Italy show. Weighted average rate on bank lending was a provisional 13.78 pct in February compared with 13.83 in January, while average weighted rate paid on deposits eased a provisional 7.49 pct from 7.66 pct. Italy today announced that its official discount rate would be cut to 11.5 pct from 12 pct effective tomorrow. REUTER \\ 
        & \textbf{\textcolor{red}{[neg] [2]}} Italy's banking industry saw an increase in the average mortgage interest rates last quarter, registering at 2.15 pct higher than the previous period. Savings account rates concurrently rose to 1.5 pct, reflecting a trend in the stabilizing economic environment. \\ 
        & \textbf{\textcolor{red}{[neg] [3]}} Italy's central bank reported an unexpected rise in the consumer price index, now standing at 5.3 pct compared to the previous 5.1 pct. This could signal higher inflation rates ahead, influencing future monetary policy decisions and potentially affecting savings account interest rates across the country. \\ 
        & \textbf{\textcolor{red}{[neg] [4]}} The Italian Treasury successfully raised 2.5 trillion lire through a private placement of short-term bonds, with significant interest from both domestic and international investors. The offering included various maturities, highlighting strong market confidence. \\
        & \textbf{\textcolor{red}{[neg] [5]}} Despite a competitive market for investment opportunities, the European Central Bank's latest report suggests that yields on fixed-rate government bonds may experience fluctuations, reflecting uncertainties in the fiscal policies of several Eurozone countries. \\ \midrule \midrule
        Llama3 info. & The European Central Bank's decision to cut its main refinancing operations rate by 10 basis points to 0.5\% has had a positive impact on Italian banks' profitability. The lower discount rate has reduced borrowing costs for lenders, allowing them to increase their lending activities and boost their earnings. For instance, UniCredit reported a 12\% rise in net income in the first quarter of 2023 compared to the same period last year, citing the benefits of the ECB's monetary policy decisions. Additionally, Intesa Sanpaolo saw its net profit increase by 15\% in the same period, attributing it to the lower interest rates. Overall, the lower discount rate has contributed to an improvement in the financial performance of Italian banks. \\ \midrule
        Llama3-dpo info. & Italy's central bank announced a surprise decision to cut its benchmark discount rate by 25 basis points on Friday, sending shockwaves through the country's financial markets. The move was widely expected to boost economic growth, but analysts are now assessing the impact on local bank earnings.The lower discount rate is likely to benefit Italian banks by reducing their borrowing costs and improving their net interest margins. UniCredit, Italy's largest lender, reported a 12\% increase in profits in the first quarter, citing improved loan demand and reduced funding costs. Other major banks, including Intesa Sanpaolo and Banco BPM, also saw their earnings rise during the period.\newline
        However, not all banks may benefit equally from the rate cut. Smaller regional lenders with higher exposure to domestic assets may struggle to pass on the reduced borrowing costs to customers, potentially limiting their ability to improve profitability. Additionally, some analysts warn that the rate cut could lead to increased competition for deposits, further eroding already thin profit margins.\newline
        Despite these concerns, most analysts expect Italy's banking sector to benefit from the lower discount rate over the medium term. A weaker euro against the dollar has also helped to support exports and stabilize the country's fragile economy, providing a positive backdrop for local banks. With the European Central Bank signaling no immediate plans to follow suit with a similar rate cut, Italy's banks are poised to reap the benefits of their country's more accommodative monetary policy stance. \\
        \midrule \midrule
        Contriever & \textbf{\textcolor{red}{[2]}} > \textbf{\textcolor{red}{[3]}} > \textbf{\textcolor{red}{[4]}} > \textbf{\textcolor{darkgreen}{[1]}} > \textbf{\textcolor{red}{[5]}} \\ \midrule
        Contriever \textbullet{} Llama3 & \textbf{\textcolor{red}{[2]}} > \textbf{\textcolor{red}{[3]}} > \textbf{\textcolor{red}{[4]}} > \textbf{\textcolor{red}{[5]}} > \textbf{\textcolor{darkgreen}{[1]}} \\ \midrule
        Contriever \textbullet{} Llama3-dpo & \textbf{\textcolor{red}{[3]}} > \textbf{\textcolor{red}{[2]}} > \textbf{\textcolor{red}{[4]}} > \textbf{\textcolor{darkgreen}{[1]}} > \textbf{\textcolor{red}{[5]}} \\ \midrule
        Contriever-st \textbullet{} Llama3 & \textbf{\textcolor{red}{[2]}} > \textbf{\textcolor{darkgreen}{[1]}} > \textbf{\textcolor{red}{[3]}} > \textbf{\textcolor{red}{[4]}} > \textbf{\textcolor{red}{[5]}} \\ \midrule
        Contriever-st \textbullet{} Llama3-dpo & \textbf{\textcolor{darkgreen}{[1]}} > \textbf{\textcolor{red}{[2]}} > \textbf{\textcolor{red}{[3]}} > \textbf{\textcolor{red}{[4]}} > \textbf{\textcolor{red}{[5]}} \\
        \bottomrule
    \end{tabularx}
    \label{case2}
    \caption{The analysis of the retrieval case.}
\end{table*}

==> related.tex <==
\section{Related Work}

\subsection{Zero-shot Retrieval.}

% introduction of zero-shot retrieval
Since domain-specific retrieval tasks often involve only a pre-existing corpus, the process of manually creating labeled supervised query-document pairs is both time-consuming and expansive \cite{thakur2021beir}. As a result, retrieval models are often applied directly to new tasks without task-specific training, a process known as zero-shot retrieval. This demands models with exceptional semantic comprehension and strong generalization abilities. The BEIR \cite{thakur2021beir} and AIR-Bench \cite{chen2024air} datasets are utilized as benchmarks to evaluate a model's zero-shot performance, assessing its effectiveness on novel tasks without prior fine-tuning for these specific tasks. However, most models exhibit restricted generalization capabilities when faced with zero-shot retrieval, which requires the incorporation of additional techniques to improve their performance \cite{gao2022precise, wang2021gpl}.

\subsection{Generation Augmented Retrieval.}

An effective method to enhance the performance of retrieval models in new tasks is Generation Augmented Retrieval (GAR), which leverages a generator to create supplementary information that strengthens retrieval. Doc2Query \cite{nogueira2019document} utilizes a generator to augment the corpus by generating potential user queries for each document and appending them to the document, thereby enriching the document's representation. HyDE \cite{gao2022precise} generates hypothetical documents from the query using a generator and employs these hypothetical documents to retrieve real documents.

However, Doc2Query processes the entire corpus, it can be more resource-intensive than producing labeling data, especially for large datasets. Moreover, changing the structure of the original document may negatively affect the performance of well-trained retrievers. In HyDE, the generation and retrieval tasks are mismatched, as the generator focuses solely on the generation process rather than creating information specifically tailored to the retrieval model's requirements. This results in a mismatch between the generated content and its intended use in retrieval.
IR-Studio is based on HyDE and trained through feedback from the retriever, effectively bridging the gap between generated information and retrieval requirements.

\subsection{Synthetic Question Generation.}

Another approach to enhance a model's performance on new tasks is by generating synthetic questions to serve as pseudo labels for training. In QGen \cite{ma2020zero}, synthetic questions are employed for training; however, these generated synthetic questions might not match the document from which they were derived. This mismatch can result in inaccurate questions or documents that aren't the gold labels for the synthetic questions. Consequently, GPL \cite{wang2021gpl} proposes scoring the generated question-document pairs using a cross-encoder as a teacher model. This scoring process helps distill the retriever's training and mitigates the impact of false positive documents, ultimately enhancing the model's performance. Nonetheless, relying solely on a cross-encoder to score query-document pairs in a new task might still yield inaccuracies, and the pseudo label quality may remain suboptimal, offering limited enhancement to the model. IR-Studio integrates the retriever and generator, efficiently utilizing generated data. Even if the labels are not of high quality, the collaborative framework yields improvements. Furthermore, IR-Studio's ranking results derive from the visibility of the generator across all documents, ensuring the efficacy of the teacher model's ranking in new tasks.
